Ricci Flow and the Poincare Conjecture

This manuscript contains a detailed proof of the Poincare Conjecture. The arguments we present here are expanded versions of the ones given by Perelman in his three preprints posted in 2002 and 2003. This is a revised version taking in account the comments of the referees and others. It has been reformatted in the AMS book style.

==> temp.tex <==
 This manuscript contains a detailed proof of the Poincare Conjecture. The
arguments we present here are expanded versions of the ones given by Perelman
in his three preprints posted in 2002 and 2003. This is a revised version
taking in account the comments of the referees and others. It has been
reformatted in the AMS book style.


493 pages with over 30 figures and 3 pages of front material

